The Design and Implementation of Typed Scheme: From Scripts to Programs

When scripts in untyped languages grow into large programs, maintaining them becomes difficult. A lack of explicit type annotations in typical scripting languages forces programmers to must (re)discover critical pieces of design information every time they wish to change a program. This analysis step both slows down the maintenance process and may even introduce mistakes due to the violation of undiscovered invariants. This paper presents Typed Scheme, an explicitly typed extension of PLT Scheme, an untyped scripting language. Its type system is based on the novel notion of occurrence typing, which we formalize and mechanically prove sound. The implementation of Typed Scheme additionally borrows elements from a range of approaches, including recursive types, true unions and subtyping, plus polymorphism combined with a modicum of local inference. The formulation of occurrence typing naturally leads to a simple and expressive version of predicates to describe refinement types. A Typed Scheme program can use these refinement types to keep track of arbitrary classes of values via the type system. Further, we show how the Typed Scheme type system, in conjunction with simple recursive types, is able to encode refinements of existing datatypes, thus expressing both proposed variations of refinement types.

==> NOHIDEZ0paper.tex <==

\input{sample.sty}

\title{The Design and Implementation of Typed Scheme: \\
From Scripts to
  Programs\footnote{This is a revised and extended version of a paper
    presented at the 35th ACM SIGPLAN-SIGACT Symposium on Principles
    of Programming Languages, 2008.  The authors were supported by
    the NSF, the USAF, and the Mozilla Foundation.}}

\titlerunning{The Design and Implementation of Typed Scheme}        %

\author{Sam Tobin-Hochstadt         \and
        Matthias Felleisen %
}

%

\institute{S. Tobin-Hochstadt \at
              Northeastern University \\
              \email{samth@ccs.neu.edu}
           \and
           M. Felleisen \at
           Northeastern University
}

\date{Received: date / Accepted: date}
%


\maketitle

\begin{abstract}
When scripts in untyped languages grow into large programs, maintaining
 them becomes difficult. A lack of explicit 
 type annotations in typical scripting languages forces programmers to must
 (re)discover critical pieces of design information every time they wish to
 change a program. This analysis step both slows down the maintenance
 process and may even introduce mistakes due to the violation of
 undiscovered invariants. 

 This paper presents Typed Scheme, an explicitly typed extension of
 PLT
 Scheme, an
 untyped scripting language. Its type system is based on the novel notion
 of \emph{occurrence typing}, which we formalize and mechanically prove
 sound. The implementation of Typed Scheme additionally borrows elements
 from a range of approaches, including recursive types, true unions and
 subtyping, plus polymorphism combined with a modicum of local
 inference.

 The formulation of occurrence typing naturally leads to a simple and
 expressive version of predicates to describe \emph{refinement types}. 
%
 A Typed Scheme program can use these refinement types to keep track
 of arbitrary classes of values via the type system.  
%
Further, we show how the Typed Scheme type system, in conjunction with
simple recursive types, is able to encode refinements of existing
datatypes, thus expressing \emph{both} proposed variations of
refinement types.   
%
%
%
%
%


\keywords{Scheme \and Type Systems \and Refinement types}
%
%
\end{abstract}

%

\input{intro.tex}

%
\input{overview.tex}

\input{extended-example}

%
\input{formal.tex}

\input{refinement.tex}

\input{scaling.tex}

\input{implementation.tex}

\input{exp.tex}

\input{related.tex}

%
\input{future.tex}


==> NOHIDEZ100paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ101paper.tex <==
\ZZZZschemecodeintext
\va{odd?}%
\endZZZZschemecodeintext


==> NOHIDEZ102paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ103paper.tex <==
\ZZZZschemecodeintext
\va{odd?}%
\endZZZZschemecodeintext


==> NOHIDEZ104paper.tex <==
\begin{ZZZZschemedisplay}%
(\l ([\va{f} \sy{:} ((\sy{Refinement} \va{even?} \sy{Number}) $\to$ \sy{Number})] [\va{n} \sy{:} \sy{Number}])\\%
\PRN \HL (\sy{if} (\va{even?} \va{n}) (\va{f} \va{n}) \va{n}))
\end{ZZZZschemedisplay}


==> NOHIDEZ105paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ106paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define:} (\va{a} \va{b}) (\va{map} [\va{f} \sy{:} (\va{a} $\to$ \va{b})] [\va{l} \sy{:} (\sy{Listof} \va{a})]) \sy{:} (\sy{Listof} \va{b})\\%
\PRN \HL \=(\sy{if} \=(\va{null?} \va{l}) \va{l}\\%
  \>    \>(\va{cons} (\va{f} (\va{car} \va{l})) (\va{map} \va{f} (\va{cdr} \va{l})))))
\end{ZZZZschemedisplay}


==> NOHIDEZ107paper.tex <==
\ZZZZschemecodeintext
\va{a}%
\endZZZZschemecodeintext


==> NOHIDEZ108paper.tex <==
\ZZZZschemecodeintext
\va{b}%
\endZZZZschemecodeintext


==> NOHIDEZ109paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ10paper.tex <==
\ZZZZschemecodeintext
\va{list-of-shapes}%
\endZZZZschemecodeintext


==> NOHIDEZ110paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ111paper.tex <==
\ZZZZschemecodeintext
\va{a}%
\endZZZZschemecodeintext


==> NOHIDEZ112paper.tex <==
\ZZZZschemecodeintext
\va{b}%
\endZZZZschemecodeintext


==> NOHIDEZ113paper.tex <==
\ZZZZschemecodeintext
\va{cons}%
\endZZZZschemecodeintext


==> NOHIDEZ114paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type-alias} \va{STree} ($\mu$ \va{t} (\ma{\bigcup} \sy{Number} (\va{cons} \va{t} \va{t}))))
\end{ZZZZschemedisplay}


==> NOHIDEZ115paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define:} (\va{sum-tree} [\va{s} \sy{:} \va{STree}]) \sy{:} \sy{Number}\\%
\PRN \HL \=(\sy{cond} \=[(\va{number?} \va{s}) \va{s}]\\%
  \>      \>[\sy{else} (\va{$+$} (\va{sum-tree} (\va{car} \va{s})) (\va{sum-tree} (\va{cdr} \va{s})))]))
\end{ZZZZschemedisplay}


==> NOHIDEZ116paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define:} (\va{m} [\va{z} \sy{:} \sy{Number}]) \sy{:} \sy{Number}\\%
\PRN \HL \=(\sy{let$\ast$} \=(\=[\va{x} \va{z}]\\%
  \>      \> \>[\va{y} (\va{$\ast$} \va{x} \va{x})])\\%
  \>\HL \HL ($-$ \va{y} \dt{1})))
\end{ZZZZschemedisplay}


==> NOHIDEZ117paper.tex <==
\ZZZZschemecodeintext
\sy{let$\ast$}%
\endZZZZschemecodeintext


==> NOHIDEZ118paper.tex <==
\ZZZZschemecodeintext
\va{x}%
\endZZZZschemecodeintext


==> NOHIDEZ119paper.tex <==
\ZZZZschemecodeintext
\va{y}%
\endZZZZschemecodeintext


==> NOHIDEZ11paper.tex <==
\ZZZZschemecodeintext
\va{rectangle}%
\endZZZZschemecodeintext


==> NOHIDEZ120paper.tex <==
\ZZZZschemecodeintext
\sy{Number}%
\endZZZZschemecodeintext


==> NOHIDEZ121paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define:} (\va{m} [\va{z} \sy{:} \sy{Number}]) \sy{:} \sy{Number}\\%
\PRN \HL \=(\sy{define} \va{x} \va{z})\\%
  \>(\sy{define} \va{y} (\va{$\ast$} \va{x} \va{x}))\\%
  \>($-$ \va{y} \dt{1}))
\end{ZZZZschemedisplay}


==> NOHIDEZ122paper.tex <==
\ZZZZschemecodeintext
\sy{letrec}%
\endZZZZschemecodeintext


==> NOHIDEZ123paper.tex <==
\ZZZZschemecodeintext
\sy{letrec}%
\endZZZZschemecodeintext


==> NOHIDEZ124paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ125paper.tex <==
\begin{ZZZZschemedisplay}%
(\va{map} (\va{lambda:} ([\va{x} \sy{:} \sy{Number}]) (\va{$+$} \va{x} \dt{1})) '(\cn{1} \cn{2} \cn{3}))
\end{ZZZZschemedisplay}


==> NOHIDEZ126paper.tex <==
\ZZZZschemecodeintext
(\sy{Number} $\to$ \sy{Number})%
\endZZZZschemecodeintext


==> NOHIDEZ127paper.tex <==
\ZZZZschemecodeintext
(\sy{Listof} \sy{Number})%
\endZZZZschemecodeintext


==> NOHIDEZ128paper.tex <==
\ZZZZschemecodeintext
(\sy{All} (\va{a} \va{b}) ((\va{a} $\to$ \va{b}) (\sy{Listof} \va{a}) $\to$ (\sy{Listof} \va{b})))%
\endZZZZschemecodeintext


==> NOHIDEZ129paper.tex <==
\begin{ZZZZschemedisplay}%
(\va{map} (\va{lambda:} ([\va{x} \sy{:} \sy{Any}]) \va{x}) '(\cn{1} \cn{2} \cn{3}))
\end{ZZZZschemedisplay}


==> NOHIDEZ12paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ130paper.tex <==
\ZZZZschemecodeintext
(\sy{Listof} \sy{Number})%
\endZZZZschemecodeintext


==> NOHIDEZ131paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ132paper.tex <==
\ZZZZschemecodeintext
\va{b}%
\endZZZZschemecodeintext


==> NOHIDEZ133paper.tex <==
\ZZZZschemecodeintext
\sy{Number}%
\endZZZZschemecodeintext


==> NOHIDEZ134paper.tex <==
\ZZZZschemecodeintext
(\sy{Any} $\to$
\sy{Any})%
\endZZZZschemecodeintext


==> NOHIDEZ135paper.tex <==
\ZZZZschemecodeintext
\va{a}%
\endZZZZschemecodeintext


==> NOHIDEZ136paper.tex <==
\ZZZZschemecodeintext
\va{b}%
\endZZZZschemecodeintext


==> NOHIDEZ137paper.tex <==
\ZZZZschemecodeintext
\sy{Any}%
\endZZZZschemecodeintext


==> NOHIDEZ138paper.tex <==
\ZZZZschemecodeintext
\sy{Number}%
\endZZZZschemecodeintext


==> NOHIDEZ139paper.tex <==
\ZZZZschemecodeintext
\sy{Any}%
\endZZZZschemecodeintext


==> NOHIDEZ13paper.tex <==
\ZZZZschemecodeintext
\va{rectangle}%
\endZZZZschemecodeintext


==> NOHIDEZ140paper.tex <==
\ZZZZschemecodeintext
\va{a}%
\endZZZZschemecodeintext


==> NOHIDEZ141paper.tex <==
\ZZZZschemecodeintext
\va{foldl}%
\endZZZZschemecodeintext


==> NOHIDEZ142paper.tex <==
\ZZZZschemecodeintext
\sy{Number}%
\endZZZZschemecodeintext


==> NOHIDEZ143paper.tex <==
\ZZZZschemecodeintext
\sy{Any}%
\endZZZZschemecodeintext


==> NOHIDEZ144paper.tex <==
\ZZZZschemecodeintext
\va{structure}%
\endZZZZschemecodeintext


==> NOHIDEZ145paper.tex <==
\ZZZZschemecodeintext
\sy{define-struct}%
\endZZZZschemecodeintext


==> NOHIDEZ146paper.tex <==
\ZZZZschemecodeintext
\sy{define-struct:}%
\endZZZZschemecodeintext


==> NOHIDEZ147paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-struct} \va{A} (\va{x} \va{y}))
\end{ZZZZschemedisplay}


==> NOHIDEZ148paper.tex <==
\ZZZZschemecodeintext
\va{A}%
\endZZZZschemecodeintext


==> NOHIDEZ149paper.tex <==
\ZZZZschemecodeintext
\va{x}%
\endZZZZschemecodeintext


==> NOHIDEZ14paper.tex <==
\ZZZZschemecodeintext
\va{scene$+$rectangle}%
\endZZZZschemecodeintext


==> NOHIDEZ150paper.tex <==
\ZZZZschemecodeintext
\va{y}%
\endZZZZschemecodeintext


==> NOHIDEZ151paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-struct:} \va{A} ([\va{x} \sy{:} \sy{Number}] [\va{y} \sy{:} \sy{String}]))
\end{ZZZZschemedisplay}


==> NOHIDEZ152paper.tex <==
\ZZZZschemecodeintext
\sy{define-struct:}%
\endZZZZschemecodeintext


==> NOHIDEZ153paper.tex <==
\ZZZZschemecodeintext
\sy{define-struct}%
\endZZZZschemecodeintext


==> NOHIDEZ154paper.tex <==
\ZZZZschemecodeintext
\va{A?}%
\endZZZZschemecodeintext


==> NOHIDEZ155paper.tex <==
\ZZZZschemecodeintext
\va{A}%
\endZZZZschemecodeintext


==> NOHIDEZ156paper.tex <==
\ZZZZschemecodeintext
\sy{define-struct:}%
\endZZZZschemecodeintext


==> NOHIDEZ157paper.tex <==
\ZZZZschemecodeintext
\sy{case-lambda}%
\endZZZZschemecodeintext


==> NOHIDEZ158paper.tex <==
\ZZZZschemecodeintext
\sy{values}%
\endZZZZschemecodeintext


==> NOHIDEZ159paper.tex <==
\ZZZZschemecodeintext
\sy{values}%
\endZZZZschemecodeintext


==> NOHIDEZ15paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ160paper.tex <==
\ZZZZschemecodeintext
\va{apply}%
\endZZZZschemecodeintext


==> NOHIDEZ161paper.tex <==
\ZZZZschemecodeintext
\va{apply}%
\endZZZZschemecodeintext


==> NOHIDEZ162paper.tex <==
\ZZZZschemecodeintext
\va{apply}%
\endZZZZschemecodeintext


==> NOHIDEZ163paper.tex <==
\ZZZZschemecodeintext
\va{apply}%
\endZZZZschemecodeintext


==> NOHIDEZ164paper.tex <==
\ZZZZschemecodeintext
\va{$+$}%
\endZZZZschemecodeintext


==> NOHIDEZ165paper.tex <==
\ZZZZschemecodeintext
(\va{apply} \va{$+$} (\va{list} \dt{1} \dt{2} \dt{3} \dt{4}))%
\endZZZZschemecodeintext


==> NOHIDEZ166paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ167paper.tex <==
\ZZZZschemecodeintext
\va{call/cc}%
\endZZZZschemecodeintext


==> NOHIDEZ168paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ169paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ16paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ170paper.tex <==
\ZZZZschemecodeintext
\va{p?}%
\endZZZZschemecodeintext


==> NOHIDEZ171paper.tex <==
\ZZZZschemecodeintext
\va{p?}%
\endZZZZschemecodeintext


==> NOHIDEZ172paper.tex <==
\begin{ZZZZschemedisplay}%
\va{filter} \sy{:} (\sy{All} (\va{a} \va{b}) ((\va{a} \ma{\stackrel{b}{\to}} \sy{Boolean}) (\sy{Listof} \va{a}) $\to$ (\sy{Listof} \va{b}))
\end{ZZZZschemedisplay}


==> NOHIDEZ173paper.tex <==
\ZZZZschemecodeintext
(\va{a} \ma{\stackrel{b}{\to}} \sy{Boolean})%
\endZZZZschemecodeintext


==> NOHIDEZ174paper.tex <==
\ZZZZschemecodeintext
\va{a}%
\endZZZZschemecodeintext


==> NOHIDEZ175paper.tex <==
\ZZZZschemecodeintext
\sy{Boolean}%
\endZZZZschemecodeintext


==> NOHIDEZ176paper.tex <==
\ZZZZschemecodeintext
\va{b}%
\endZZZZschemecodeintext


==> NOHIDEZ177paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define:} \va{the-numbers} (\sy{Listof} \sy{Number})\\%
\PRN \HL \=(\sy{let} ([\va{lst} (\va{list} '\cn{a} \dt{1} '\cn{b} \dt{2} '\cn{c} \dt{3})])\\%
  \>\PRN \HL (\va{map} \va{add1} (\va{filter} \va{number?} \va{lst}))))
\end{ZZZZschemedisplay}


==> NOHIDEZ178paper.tex <==
\ZZZZschemecodeintext
\va{the-numbers}%
\endZZZZschemecodeintext


==> NOHIDEZ179paper.tex <==
\ZZZZschemecodeintext
(\sy{Listof} \sy{Number})%
\endZZZZschemecodeintext


==> NOHIDEZ17paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ180paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ181paper.tex <==
\ZZZZschemecodeintext
\va{filter}%
\endZZZZschemecodeintext


==> NOHIDEZ182paper.tex <==
\ZZZZschemecodeintext
\va{call/cc}%
\endZZZZschemecodeintext


==> NOHIDEZ183paper.tex <==
\begin{ZZZZschemedisplay}%
\va{call/cc} \sy{:} (\sy{All} (\va{a}) (((\va{a} $\to$ \ma{\bot}) $\to$ \va{a}) $\to$ \va{a}))
\end{ZZZZschemedisplay}


==> NOHIDEZ184paper.tex <==
\ZZZZschemecodeintext
\ma{\bot}%
\endZZZZschemecodeintext


==> NOHIDEZ185paper.tex <==
\ZZZZschemecodeintext
\va{call/cc}%
\endZZZZschemecodeintext


==> NOHIDEZ186paper.tex <==
\begin{ZZZZschemedisplay}%
\ma{\#{\bf lang}} \va{typed-scheme}\\%
(\sy{provide} \va{LoN} \va{sum})\\%
(\sy{define-type-alias} \va{LoN} (\sy{Listof} \sy{Number}))\\%
(\sy{define:} (\va{sum} [\va{l} \sy{:} \va{LoN}]) \sy{:} \sy{Number}\\%
\PRN \HL (\sy{if} (\va{null?} \va{l}) \dt{0} (\va{$+$} (\va{car} \va{l}) (\va{sum} (\va{cdr} \va{l}))))))
\end{ZZZZschemedisplay}


==> NOHIDEZ187paper.tex <==
\begin{ZZZZschemedisplay}%
\ma{\#{\bf lang}} \va{typed-scheme}\\%
(\va{require} \va{m1})\\%
(\sy{define:} \va{l} \sy{:} \va{LoN} (\va{list} \dt{1} \dt{2} \dt{3} \dt{4} \dt{5}))\\%
(\va{display} (\va{sum} \va{l})))
\end{ZZZZschemedisplay}


==> NOHIDEZ188paper.tex <==
\ZZZZschemecodeintext
\va{LoN}%
\endZZZZschemecodeintext


==> NOHIDEZ189paper.tex <==
\ZZZZschemecodeintext
\va{sum}%
\endZZZZschemecodeintext


==> NOHIDEZ18paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ190paper.tex <==
\ZZZZschemecodeintext
\va{m1}%
\endZZZZschemecodeintext


==> NOHIDEZ191paper.tex <==
\ZZZZschemecodeintext
\va{m2}%
\endZZZZschemecodeintext


==> NOHIDEZ192paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{require/typed} \va{scheme} [\va{add1} (\sy{Number} $\to$ \sy{Number})])
\end{ZZZZschemedisplay}


==> NOHIDEZ193paper.tex <==
\ZZZZschemecodeintext
\va{add1}%
\endZZZZschemecodeintext


==> NOHIDEZ194paper.tex <==
\ZZZZschemecodeintext
\va{scheme}%
\endZZZZschemecodeintext


==> NOHIDEZ195paper.tex <==
\ZZZZschemecodeintext
\sy{require/typed}%
\endZZZZschemecodeintext


==> NOHIDEZ196paper.tex <==
\ZZZZschemecodeintext
\sy{require/typed}%
\endZZZZschemecodeintext


==> NOHIDEZ197paper.tex <==
\ZZZZschemecodeintext
\va{require}%
\endZZZZschemecodeintext


==> NOHIDEZ198paper.tex <==
\ZZZZschemecodeintext
(\va{number?} . $\to$ . \va{number?})%
\endZZZZschemecodeintext


==> NOHIDEZ199paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{require/typed} [\sy{opaque} \va{xml} \va{Doc} \va{document?}])
\end{ZZZZschemedisplay}


==> NOHIDEZ19paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{:} \va{just-even} (\sy{Number} $\to$ (\sy{Refinement} \va{even?})))\\%
(\sy{define} (\va{just-even} \va{n})\\%
\PRN \HL (\sy{if} (\va{even?} \va{n}) \va{n} (\va{error} '\cn{not-even})))
\end{ZZZZschemedisplay}


==> NOHIDEZ1paper.tex <==
\ZZZZschemecodeintext
\va{even?}%
\endZZZZschemecodeintext


==> NOHIDEZ200paper.tex <==
\ZZZZschemecodeintext
\va{document?}%
\endZZZZschemecodeintext


==> NOHIDEZ201paper.tex <==
\ZZZZschemecodeintext
\va{xml}%
\endZZZZschemecodeintext


==> NOHIDEZ202paper.tex <==
\ZZZZschemecodeintext
\va{Doc}%
\endZZZZschemecodeintext


==> NOHIDEZ203paper.tex <==
\ZZZZschemecodeintext
\sy{require/typed}%
\endZZZZschemecodeintext


==> NOHIDEZ204paper.tex <==
\ZZZZschemecodeintext
\va{Doc}%
\endZZZZschemecodeintext


==> NOHIDEZ205paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{module} \va{m} \va{language}\\%
\PRN \HL \HL {\dots})
\end{ZZZZschemedisplay}


==> NOHIDEZ206paper.tex <==
\ZZZZschemecodeintext
\va{language}%
\endZZZZschemecodeintext


==> NOHIDEZ207paper.tex <==
\ZZZZschemecodeintext
\sy{\#\%module-begin}%
\endZZZZschemecodeintext


==> NOHIDEZ208paper.tex <==
\ZZZZschemecodeintext
\sy{and}%
\endZZZZschemecodeintext


==> NOHIDEZ209paper.tex <==
\ZZZZschemecodeintext
\va{local-expand}%
\endZZZZschemecodeintext


==> NOHIDEZ20paper.tex <==
\ZZZZschemecodeintext
\va{cons}%
\endZZZZschemecodeintext


==> NOHIDEZ210paper.tex <==
\ZZZZschemecodeintext
\va{unit}%
\endZZZZschemecodeintext


==> NOHIDEZ211paper.tex <==
\ZZZZschemecodeintext
\va{class}%
\endZZZZschemecodeintext


==> NOHIDEZ212paper.tex <==
\ZZZZschemecodeintext
\va{class}%
\endZZZZschemecodeintext


==> NOHIDEZ213paper.tex <==
\ZZZZschemecodeintext
(\va{pair?} (\va{car} \va{x}))%
\endZZZZschemecodeintext


==> NOHIDEZ214paper.tex <==
\ZZZZschemecodeintext
\va{galore.plt}%
\endZZZZschemecodeintext


==> NOHIDEZ215paper.tex <==
\ZZZZschemecodeintext
\va{turn}%
\endZZZZschemecodeintext


==> NOHIDEZ216paper.tex <==
\ZZZZschemecodeintext
\va{player}%
\endZZZZschemecodeintext


==> NOHIDEZ217paper.tex <==
\ZZZZschemecodeintext
\sy{define}%
\endZZZZschemecodeintext


==> NOHIDEZ218paper.tex <==
\ZZZZschemecodeintext
\sy{define:}%
\endZZZZschemecodeintext


==> NOHIDEZ219paper.tex <==
\ZZZZschemecodeintext
\va{the-end}%
\endZZZZschemecodeintext


==> NOHIDEZ21paper.tex <==
\ZZZZschemecodeintext
(\va{list} \dt{1} \dt{2} \dt{3})%
\endZZZZschemecodeintext


==> NOHIDEZ220paper.tex <==
\ZZZZschemecodeintext
\va{the-return-card}%
\endZZZZschemecodeintext


==> NOHIDEZ221paper.tex <==
\ZZZZschemecodeintext
\va{res}%
\endZZZZschemecodeintext


==> NOHIDEZ222paper.tex <==
\ZZZZschemecodeintext
\va{end}%
\endZZZZschemecodeintext


==> NOHIDEZ223paper.tex <==
\ZZZZschemecodeintext
\sy{require/typed}%
\endZZZZschemecodeintext


==> NOHIDEZ224paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{:} \va{play-one-turn} \=(\va{Player} \va{Cards} \va{Cards} \va{Hand} $\to$\\%
                 \>\PRN (\sy{values} \sy{Boolean} \va{RCard} \va{Hand} \va{Attacks} \va{From}))) \\%
(\sy{define} (\va{play-one-turn} \va{player} \va{deck} \va{stck} \va{fst:discs}) \\%
\PRN \HL \=(\sy{define} \va{trn} (\va{create-turn} (\va{player-name} \va{player}) \va{deck} \va{stck} \va{fst:discs}))\\%
  \>;; --- go play \\%
  \>(\sy{define} \va{res} (\va{player-take-turn} \va{player} \va{trn}))\\%
  \>;; the-return-card could be false\\%
  \>(\sy{define-values} (\va{the-end} \va{the-return-card})\\%
  \>\PRN \HL \=(\sy{cond}\\%
  \>  \>\PRN \=[(\va{ret?} \va{res}) (\sy{values} \dt{\#f} (\va{ret-card} \va{res}))]\\%
  \>  \> \>[(\va{end?} \va{res}) (\sy{values} \dt{\#t} (\va{end-card} \va{res}))]))\\%
  \>(\sy{define} \va{discards:squadrons} \ (\va{done-discards} \va{res}))\\%
  \>(\sy{define} \va{attacks} \ (\va{done-attacks} \va{res}))\\%
  \>(\sy{define} \va{et} (\va{turn-end} \va{trn}))\\%
  \>(\sy{values} \va{the-end} \va{the-return-card} \va{discards:squadrons} \va{attacks} \va{et}))
\end{ZZZZschemedisplay}


==> NOHIDEZ225paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ226paper.tex <==
\ZZZZschemecodeintext
\va{number?}%
\endZZZZschemecodeintext


==> NOHIDEZ227paper.tex <==
\ZZZZschemecodeintext
\sy{or}%
\endZZZZschemecodeintext


==> NOHIDEZ228paper.tex <==
\ZZZZschemecodeintext
(\va{number?} \va{e})%
\endZZZZschemecodeintext


==> NOHIDEZ229paper.tex <==
\ZZZZschemecodeintext
\va{e}%
\endZZZZschemecodeintext


==> NOHIDEZ22paper.tex <==
\ZZZZschemecodeintext
(\va{cons} \sy{Number} (\va{cons} \sy{Number} (\va{cons} \sy{Number} '())))%
\endZZZZschemecodeintext


==> NOHIDEZ230paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ231paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ23paper.tex <==
\ZZZZschemecodeintext
(\sy{Listof} \sy{Number})%
\endZZZZschemecodeintext


==> NOHIDEZ24paper.tex <==
\ZZZZschemecodeintext
\sy{Listof}%
\endZZZZschemecodeintext


==> NOHIDEZ25paper.tex <==
\ZZZZschemecodeintext
\va{cons}%
\endZZZZschemecodeintext


==> NOHIDEZ26paper.tex <==
\ZZZZschemecodeintext
\va{apply}%
\endZZZZschemecodeintext


==> NOHIDEZ27paper.tex <==
\ZZZZschemecodeintext
\va{map}%
\endZZZZschemecodeintext


==> NOHIDEZ28paper.tex <==
\ZZZZschemecodeintext
\va{foldl}%
\endZZZZschemecodeintext


==> NOHIDEZ29paper.tex <==
\begin{ZZZZschemedisplay}%
(\va{string-append} \dt{{\dq}SELECT $\ast$ FROM users WHERE name $=$ '{\dq}} \va{user-name} \dt{{\dq}';{\dq}})
\end{ZZZZschemedisplay}


==> NOHIDEZ2paper.tex <==
\begin{ZZZZschemedisplay}%
;; data definition: a Complex is either \\%
;; - a Number or \\%
;; - (cons Number Number)
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
;; Complex $\rightarrow$ Number\\%
(\sy{define} (\va{creal} \va{x})\\%
\PRN \HL \=(\sy{cond} \=[(\va{number?} \va{x}) \va{x}]\\%
  \>      \>[\sy{else} (\va{car} \va{x})]))
\end{ZZZZschemedisplay}


==> NOHIDEZ30paper.tex <==
\ZZZZschemecodeintext
\va{user-name}%
\endZZZZschemecodeintext


==> NOHIDEZ31paper.tex <==
\ZZZZschemecodeintext
\dt{{\dq}a' or 't'$=$'t{\dq}}%
\endZZZZschemecodeintext


==> NOHIDEZ32paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{:} \va{sql-safe?} (\sy{String} $\to$ \sy{Boolean}))\\%
(\sy{define} (\va{sql-safe?} \va{s}) \mbox{$\mbox{\tiny ~~{\it omitted\/}~~} \over ~$})
\end{ZZZZschemedisplay}


==> NOHIDEZ33paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{declare-refinement} \va{sql-safe?})
\end{ZZZZschemedisplay}


==> NOHIDEZ34paper.tex <==
\ZZZZschemecodeintext
\va{sql-safe?}%
\endZZZZschemecodeintext


==> NOHIDEZ35paper.tex <==
\ZZZZschemecodeintext
(\sy{Refinement} \va{sql-safe?} \sy{String})%
\endZZZZschemecodeintext


==> NOHIDEZ36paper.tex <==
\ZZZZschemecodeintext
\va{sql-safe?}%
\endZZZZschemecodeintext


==> NOHIDEZ37paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{:} \va{query} ((\sy{Refinement} \va{sql-safe?} \sy{String}) $\to$ (\sy{Listof} \va{Result})))\\%
(\sy{define} (\va{query} \va{user-name})\\%
\PRN \HL \=(\va{run-query}\\%
  \>\PRN (\va{string-append} \dt{{\dq}SELECT $\ast$ FROM users WHERE name $=$ '{\dq}} \va{user-name} \dt{{\dq}';{\dq}})))
\end{ZZZZschemedisplay}


==> NOHIDEZ38paper.tex <==
\ZZZZschemecodeintext
(\sy{Refinement} \va{sql-safe?} \sy{String})%
\endZZZZschemecodeintext


==> NOHIDEZ39paper.tex <==
\ZZZZschemecodeintext
\sy{String}%
\endZZZZschemecodeintext


==> NOHIDEZ3paper.tex <==
\ZZZZschemecodeintext
\sy{cond}%
\endZZZZschemecodeintext


==> NOHIDEZ40paper.tex <==
\ZZZZschemecodeintext
\va{user-name}%
\endZZZZschemecodeintext


==> NOHIDEZ41paper.tex <==
\ZZZZschemecodeintext
\va{string-append}%
\endZZZZschemecodeintext


==> NOHIDEZ42paper.tex <==
\ZZZZschemecodeintext
\va{sanitize}%
\endZZZZschemecodeintext


==> NOHIDEZ43paper.tex <==
\ZZZZschemecodeintext
\va{sql-safe?}%
\endZZZZschemecodeintext


==> NOHIDEZ44paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{:} \va{sanitize} (\sy{String} $\to$ (\sy{Refinement} \va{sql-safe?} \sy{String})))\\%
(\sy{define} (\va{sanitize} \va{s})\\%
\PRN \HL \=(\sy{define} \va{s$\ast$} (\va{string-map} \va{escape-char} \va{s}))\\%
  \>(\sy{if} (\va{sql-safe?} \va{s}) \va{s} (\va{error} \dt{{\dq}escape failed{\dq}})))
\end{ZZZZschemedisplay}


==> NOHIDEZ45paper.tex <==
\ZZZZschemecodeintext
\va{sql-safe?}%
\endZZZZschemecodeintext


==> NOHIDEZ46paper.tex <==
\ZZZZschemecodeintext
\va{sanitize}%
\endZZZZschemecodeintext


==> NOHIDEZ47paper.tex <==
\ZZZZschemecodeintext
\va{SQLSafeString}%
\endZZZZschemecodeintext


==> NOHIDEZ48paper.tex <==
\ZZZZschemecodeintext
\va{SQLSafeString}%
\endZZZZschemecodeintext


==> NOHIDEZ49paper.tex <==
\ZZZZschemecodeintext
\va{string-append}%
\endZZZZschemecodeintext


==> NOHIDEZ4paper.tex <==
\ZZZZschemecodeintext
\va{x}%
\endZZZZschemecodeintext


==> NOHIDEZ50paper.tex <==
\ZZZZschemecodeintext
\sy{Integer}%
\endZZZZschemecodeintext


==> NOHIDEZ51paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type} \va{IntList} (\sy{Rec} \va{L} (\ma{\bigcup} '() (\sy{Pair} \sy{Integer} \va{L}))))
\end{ZZZZschemedisplay}


==> NOHIDEZ52paper.tex <==
\ZZZZschemecodeintext
\sy{Rec}%
\endZZZZschemecodeintext


==> NOHIDEZ53paper.tex <==
\ZZZZschemecodeintext
'()%
\endZZZZschemecodeintext


==> NOHIDEZ54paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type} \va{NonEmpty} (\sy{Pair} \sy{Integer} (\sy{Rec} \va{L} (\ma{\bigcup} '() (\sy{Pair} \sy{Integer} \va{L}))))
\end{ZZZZschemedisplay}


==> NOHIDEZ55paper.tex <==
\ZZZZschemecodeintext
\va{NonEmpty}%
\endZZZZschemecodeintext


==> NOHIDEZ56paper.tex <==
\ZZZZschemecodeintext
\va{IntList}%
\endZZZZschemecodeintext


==> NOHIDEZ57paper.tex <==
\ZZZZschemecodeintext
$V_u$%
\endZZZZschemecodeintext


==> NOHIDEZ58paper.tex <==
\ZZZZschemecodeintext
$V_k$%
\endZZZZschemecodeintext


==> NOHIDEZ59paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type} $V_u$ \sy{Symbol})\\%
(\sy{define-struct:} $V_k$ ([\va{v} \sy{:} \sy{Symbol}]))\\%
(\sy{define-type} $V$ (\ma{\bigcup} $V_u$ $V_k$))
\end{ZZZZschemedisplay}


==> NOHIDEZ5paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type-alias} \va{Cplx} (\ma{\bigcup} \sy{Number} (\va{cons} \sy{Number} \sy{Number})))
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
(\sy{define:} (\va{creal} [\va{x} \sy{:} \va{Cplx}]) \sy{:} \sy{Number}\\%
\PRN \HL \=(\sy{cond} \=[(\va{number?} \va{x}) \va{x}]\\%
  \>      \>[\sy{else} (\va{car} \va{x})]))
\end{ZZZZschemedisplay}


==> NOHIDEZ60paper.tex <==
\ZZZZschemecodeintext
$\lambda$%
\endZZZZschemecodeintext


==> NOHIDEZ61paper.tex <==
\ZZZZschemecodeintext
\va{app}%
\endZZZZschemecodeintext


==> NOHIDEZ62paper.tex <==
\ZZZZschemecodeintext
$\lambda$%
\endZZZZschemecodeintext


==> NOHIDEZ63paper.tex <==
\ZZZZschemecodeintext
\va{app}%
\endZZZZschemecodeintext


==> NOHIDEZ64paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-struct:} (\va{V} \va{A}) $\lambda$ ([\va{x} \sy{:} \va{V}] [\va{b} \sy{:} \va{A}]))\\%
(\sy{define-struct:} (\va{A} \va{B}) \va{app} ([\va{rator} \sy{:} \va{A}] [\va{rand} \sy{:} \va{B}]))
\end{ZZZZschemedisplay}


==> NOHIDEZ65paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type} ($\lambda_{U}$ \va{A}) ($\lambda$ $V_u$ \va{A}))\\%
(\sy{define-type} ($\lambda_{K}$ \va{A}) ($\lambda$ $V_k$ \va{A}))\\%
(\sy{define-type} ($\lambda_A$ \va{A}) ($\lambda$ $V$ \va{A}))
\end{ZZZZschemedisplay}


==> NOHIDEZ66paper.tex <==
\ZZZZschemecodeintext
$\lambda_{U}$%
\endZZZZschemecodeintext


==> NOHIDEZ67paper.tex <==
\ZZZZschemecodeintext
$\lambda_{K}$%
\endZZZZschemecodeintext


==> NOHIDEZ68paper.tex <==
\ZZZZschemecodeintext
$\lambda_A$%
\endZZZZschemecodeintext


==> NOHIDEZ69paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{define-type} $\Lambda$ (\sy{Rec} \va{L} (\ma{\bigcup} $V$ ($\lambda_A$ \va{L}) (\va{app} \va{L} \va{L}))))
\end{ZZZZschemedisplay}


==> NOHIDEZ6paper.tex <==
\ZZZZschemecodeintext
\va{Cplx}%
\endZZZZschemecodeintext


==> NOHIDEZ70paper.tex <==
\ZZZZschemecodeintext
$V$%
\endZZZZschemecodeintext


==> NOHIDEZ71paper.tex <==
We can write these definitions directly as Typed Scheme types:%
\footnote{Unfortunately, Typed Scheme currently requires the
  equivalent, but more verbose definition of \ZZZZschemecodeintext
\va{P}%
\endZZZZschemecodeintext{} and
  \ZZZZschemecodeintext
\va{K}%
\endZZZZschemecodeintext{}, in which the other definitions are inlined:
\begin{ZZZZschemedisplay}%
(\sy{define-type} \va{P} (\va{app} \va{K} (\ma{\bigcup} $V_u$ ($\lambda_{K}$ \va{K}))))\\%
(\sy{define-type} \va{K} (\sy{Rec} \va{K} (\ma{\bigcup} $V_k$ (\va{app} (\ma{\bigcup} $V_u$ ($\lambda_{K}$ \va{K})) \va{K}) ($\lambda_{U}$ (\va{app} \va{K} (\ma{\bigcup} $V_u$ ($\lambda_{K}$ \va{K})))))))
\end{ZZZZschemedisplay}
We are investigating how to admit the shorter syntax directly.}
\begin{ZZZZschemedisplay}%
(\sy{define-type} \va{P} (\va{app} \va{K} \va{W}))\\%
(\sy{define-type} \va{W} (\ma{\bigcup} $V_u$ ($\lambda_{K}$ \va{K})))\\%
(\sy{define-type} \va{K} (\ma{\bigcup} $V_k$ (\va{app} \va{W} \va{K}) ($\lambda_{K}$ \va{K}))
\end{ZZZZschemedisplay}
All of the types are of course subtypes of \ZZZZschemecodeintext
$\Lambda$%
\endZZZZschemecodeintext{}.  Thus,
compiler writers can
write typeful functions that manipulate CPS terms, while also
using more general functions that accept arbitrary terms (such as evaluators) on them.

==> NOHIDEZ72paper.tex <==
\ZZZZschemecodeintext
\ma{\bot}%
\endZZZZschemecodeintext


==> NOHIDEZ73paper.tex <==
\begin{ZZZZschemedisplay}%
(\l (\va{x} \sy{:} (\ma{\bigcup} \sy{Number} \sy{Boolean})) \\%
\PRN \HL (\sy{if} (\va{number?} \va{x}) (\va{$=$} \va{x} \dt{1}) (\va{not} \va{x})))
\end{ZZZZschemedisplay}


==> NOHIDEZ74paper.tex <==
\ZZZZschemecodeintext
\sy{Number}%
\endZZZZschemecodeintext


==> NOHIDEZ75paper.tex <==
\ZZZZschemecodeintext
\va{x}%
\endZZZZschemecodeintext


==> NOHIDEZ76paper.tex <==
\ZZZZschemecodeintext
\sy{Boolean}%
\endZZZZschemecodeintext


==> NOHIDEZ77paper.tex <==
\ZZZZschemecodeintext
(\ma{\bigcup} \sy{Number} \sy{Boolean})%
\endZZZZschemecodeintext


==> NOHIDEZ78paper.tex <==
\ZZZZschemecodeintext
\va{procedure?}%
\endZZZZschemecodeintext


==> NOHIDEZ79paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{if} (\va{number?} \va{x}) \dt{\#t} (\va{boolean?} \va{x}))
\end{ZZZZschemedisplay}


==> NOHIDEZ7paper.tex <==
\ZZZZschemecodeintext
\va{creal}%
\endZZZZschemecodeintext


==> NOHIDEZ80paper.tex <==
\ZZZZschemecodeintext
\va{bool-or-number}%
\endZZZZschemecodeintext


==> NOHIDEZ81paper.tex <==
\begin{ZZZZschemedisplay}%
(\l (\va{x} \sy{:} \sy{Any}) (\sy{if} (\va{number?} \va{x}) \dt{\#t} (\va{boolean?} \va{x})))
\end{ZZZZschemedisplay}


==> NOHIDEZ82paper.tex <==
\ZZZZschemecodeintext
(\sy{Any} \ma{\stackrel{\mbox{(\usym\ {\bf Number} {\bf Boolean})}}{\to}} \sy{Boolean})%
\endZZZZschemecodeintext


==> NOHIDEZ83paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ84paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ85paper.tex <==
\ZZZZschemecodeintext
\va{bool-or-number}%
\endZZZZschemecodeintext


==> NOHIDEZ86paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ87paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ88paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{if} (\va{number?} \va{x}) \dt{\#t} (\va{boolean?} \va{x}))
\end{ZZZZschemedisplay}


==> NOHIDEZ89paper.tex <==
\ZZZZschemecodeintext
\sy{or}%
\endZZZZschemecodeintext


==> NOHIDEZ8paper.tex <==
\begin{ZZZZschemedisplay}%
(\va{foldl} \va{scene$+$rectangle} \va{empty-scene} (\va{filter} \va{rectangle?} \va{list-of-shapes}))
\end{ZZZZschemedisplay}


==> NOHIDEZ90paper.tex <==
\begin{ZZZZschemedisplay}%
(\l (\va{x} \sy{:} (\ma{\bigcup} \sy{Number} \sy{Boolean})) (\sy{if} (\va{number?} \va{x}) (\va{$=$} \va{x} \dt{1}) (\va{not} \va{x})))
\end{ZZZZschemedisplay}


==> NOHIDEZ91paper.tex <==
\ZZZZschemecodeintext
\sy{if}%
\endZZZZschemecodeintext


==> NOHIDEZ92paper.tex <==
\ZZZZschemecodeintext
\ma{\bot}%
\endZZZZschemecodeintext


==> NOHIDEZ93paper.tex <==
\ZZZZschemecodeintext
\va{procedure?}%
\endZZZZschemecodeintext


==> NOHIDEZ94paper.tex <==
\ZZZZschemecodeintext
\dt{\#f}%
\endZZZZschemecodeintext


==> NOHIDEZ95paper.tex <==
\begin{ZZZZschemedisplay}%
(\sy{if} (\va{number?} \dt{\#f}) (\va{$=$} \dt{\#f} \dt{1}) (\va{not} \dt{\#f}))
\end{ZZZZschemedisplay}


==> NOHIDEZ96paper.tex <==
\ZZZZschemecodeintext
\va{$=$}%
\endZZZZschemecodeintext


==> NOHIDEZ97paper.tex <==
\ZZZZschemecodeintext
\dt{\#t}%
\endZZZZschemecodeintext


==> NOHIDEZ98paper.tex <==
\ZZZZschemecodeintext
(\va{number?} \dt{\#f})%
\endZZZZschemecodeintext


==> NOHIDEZ99paper.tex <==
\ZZZZschemecodeintext
\dt{0}%
\endZZZZschemecodeintext


==> NOHIDEZ9paper.tex <==
\ZZZZschemecodeintext
\va{rectangle}%
\endZZZZschemecodeintext

